DB-Nets: on The Marriage of Colored Petri Nets and Relational Databases

The integrated management of business processes and mas- ter data is being increasingly considered as a fundamental problem, by both the academia and the industry. In this position paper, we focus on the foundations of the problem, arguing that contemporary approaches struggle to find a suitable equilibrium between data- and process-related aspects. We then propose db-nets, a new formal model that balances such two pillars through the marriage of colored Petri nets and relational databases. We invite the research community to build on this model, discussing its potential in modeling, formal verification, and simulation.

==> 5-conclusions.tex <==
\section{Conclusions}
We have presented a formal Petri net model, so called db-nets, allowing to describe data-enriched processes directly interacting with an underlying relational database. Db-nets offer \begin{inparaenum}[\it a)]
\item full access to results of queries ran on top of the database so to extract data critical to the Petri net flow enactment, and
\item transactional updates over the same database by calling predefined actions that are issued together with a firing transition they have been assigned to.
\end{inparaenum}



\endinput
Merging data and Petri nets was a hot topic since the Petri net community acquired high-level Petri net extensions to model complex systems

We are having a fresh look at the processes (or information systems) interacting with databases due to already existing works on data-aware processes that provide enough of theoretical results to talk about structural and behavioral properties of the systems. 

Mention dataflow languages where ppl use petri nets + nested relational calculus. In our case we use full-fledged reasoning over relational databases.

formal semantics for data-intensive workflows is usually not provided
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% save-place: t
%%% End:


==> dbnet-example.tex <==
\begin{figure}
\centering
\begin{tikzpicture}[->,>=stealth',auto,x=1.6cm,y=1.6 cm,thick]
% initialization
  \node[place,label={below,xshift=-.2cm:$START$}] (i) at (0,1) {};
  \viewplace{users}{(0,3)}{above:$\begin{array}{@{}l@{}}
                 \text{Registered}\\
  				\text{Users}
               \end{array}
               $};
  \node[transition, 
  label=below:$\begin{array}{@{}l@{}}
                 \text{log}\\
  				\text{in}
               \end{array}
               $] (login) at (1,2) {};
  \node[transition, 
  label=below:$\begin{array}{@{}l@{}}
                 \text{register}\\
  				\text{customer}
               \end{array}
               $] (new) at (1,0) {};

%normal arcs path
\path
(i) edge node[below] {}  (new)
(i) edge node[below] {} (login)
;
%view arcs
\path[-]
(users) edge node[below] {} (login)
;


\end{tikzpicture}
\caption{db-net modeling order processing workflow} \label{fig:wf-data-net}
\end{figure}
